ClusterComm: Discrete Communication in Decentralized MARL using Internal Representation Clustering

In the realm of Multi-Agent Reinforcement Learning (MARL), prevailing approaches exhibit shortcomings in aligning with human learning, robustness, and scalability. Addressing this, we introduce ClusterComm, a fully decentralized MARL framework where agents communicate discretely without a central control unit. ClusterComm utilizes Mini-Batch-K-Means clustering on the last hidden layer's activations of an agent's policy network, translating them into discrete messages. This approach outperforms no communication and competes favorably with unbounded, continuous communication and hence poses a simple yet effective strategy for enhancing collaborative task-solving in MARL.

==> content/3_related_work.tex <==
\section{RELATED WORK} \label{sec:related-work}
The coordination of independently trained agents with the ability to communicate has already been studied by Jaques et al.~\cite{jaques2019social}. At each time step, an agent simulates alternative actions it could have taken by counterfactual reasoning and calculates their effects on the behavior of other agents. Actions that lead to significant changes in the behavior of other agents are considered influential and are rewarded. However, this method assumes that an agent has access to the other agents' policies. ClusterComm does not require counterfactual simulation of actions, nor does it require access to the entire policies of all other agents.\\
The same problem is also studied by Eccles et al.~\cite{eccles2019biases}. Here, agents are explicitly regularized to produce meaningful messages (\textit{Positive Signaling}) as well as to respond to incoming messages (\textit{Positive Listening}). Such a regularization is not necessary in the proposed approach, because the type of messages is already fixed externally. The experiments demonstrate that the agents respond to the messages even without any additional incentive.\\
Our basic assumptions of a discrete, low-bandwidth communication channel is similar to~\cite{foerster2016learning,lin2021learning}. However, the authors use binary messages of various lengths ($1$ and $10$, respectively) whereas we use the one-hot encoding.\\
ClusterComm is most closely related to AEcomm~\cite{lin2021learning}. Here, agents also exchange discrete indices. But in contrast to the present work, AEcomm uses an additional autoencoder to generate messages. In this case, each agent trains its own autoencoder, which reduces the local state of the agent to a small number of activations, discretizes it using the straight-through estimator~\cite{bengio2013estimating} and subsequently reconstructs it. Hence, it is necessary to train an additional network with an additional training task here. Furthermore, the authors found that AEcomm offers only minor advantages over using the entire internal representation of the agent. Based on this finding, we developed ClusterComm. It discretizes the agents' internal representations by iterative clustering during training and transmit the cluster indices. Doing so, eliminates the need to train an additional neural network.
